ORB5: a global electromagnetic gyrokinetic code using the PIC approach in toroidal geometry

This paper presents the current state of the global gyrokinetic code ORB5 as an update of the previous reference [Jolliet et al., Comp. Phys. Commun. 177 409 (2007)]. The ORB5 code solves the electromagnetic Vlasov-Maxwell system of equations using a PIC scheme and also includes collisions and strong flows. The code assumes multiple gyrokinetic ion species at all wavelengths for the polarization density and drift-kinetic electrons. Variants of the physical model can be selected for electrons such as assuming an adiabatic response or a ``hybrid'' model in which passing electrons are assumed adiabatic and trapped electrons are drift-kinetic. A Fourier filter as well as various control variates and noise reduction techniques enable simulations with good signal-to-noise ratios at a limited numerical cost. They are completed with different momentum and zonal flow-conserving heat sources allowing for temperature-gradient and flux-driven simulations. The code, which runs on both CPUs and GPUs, is well benchmarked against other similar codes and analytical predictions, and shows good scalability up to thousands of nodes.

==> Makefile <==
#########################################################
# Compiles the LaTeX document and make the bibliography #
# $> make review   to have review version               #
# $> make preprint to have preprint version             #
# $> make final    to have final version                #
# $> make          to have all three versions           #
#########################################################

NAME     = ORB5Review
REVIEW   = $(NAME)_Review
PREPRINT = $(NAME)_PrePrint
FINAL    = $(NAME)_Final

SRC = $(NAME).tex
REF = $(NAME).bib
FIG = FIGURES

TEX = pdflatex
BIB = bibtex

.PHONY: clean

all : review #clean

review : $(SRC)
	echo "First compilation"
	echo "================================================================="
	$(TEX) -jobname=$(REVIEW) '\def\review{} \input{$(SRC)}'
	echo "Bibtex"
	echo "================================================================="
	$(BIB) $(REVIEW).aux
	echo "Second compilation"
	echo "================================================================="
	$(TEX) -jobname=$(REVIEW) '\def\review{} \input{$(SRC)}'
	echo "Third compilation"
	echo "================================================================="
	$(TEX) -jobname=$(REVIEW) '\def\review{} \input{$(SRC)}'

preprint : $(SRC)
	$(TEX) -jobname=$(PREPRINT) '\def\preprint{} \input{$(SRC)}'
	$(BIB) $(PREPRINT).aux
	$(TEX) -jobname=$(PREPRINT) '\def\preprint{} \input{$(SRC)}'
	$(TEX) -jobname=$(PREPRINT) '\def\preprint{} \input{$(SRC)}'

final : $(SRC)
	$(TEX) -jobname=$(FINAL) '\def\final{} \input{$(SRC)}'
	$(BIB) $(FINAL).aux
	$(TEX) -jobname=$(FINAL) '\def\final{} \input{$(SRC)}'
	$(TEX) -jobname=$(FINAL) '\def\final{} \input{$(SRC)}'

clean :
	rm -f *.blg *.bbl *.spl *.aux *.out *.log *.toc

distclean : clean
	rm -f $(FIG)/*converted*
	rm -f *.pdf

